Efficient Gate Reordering for Distributed Quantum Compiling in Data Centers

Just as classical computing relies on distributed systems, the quantum computing era requires new kinds of infrastructure and software tools. Quantum networks will become the backbone of hybrid, quantum-augmented data centers, in which quantum algorithms are distributed over a local network of quantum processing units (QPUs) interconnected via shared entanglement. In this context, it is crucial to develop methods and software that minimize the number of inter-QPU communications. Here we describe key features of the quantum compiler araQne, which is designed to minimize distribution cost, measured by the number of entangled pairs required to distribute a monolithic quantum circuit using gate teleportation protocols. We establish the crucial role played by circuit reordering strategies, which strongly reduce the distribution cost compared to a baseline approach.

==> drawings/distributed.tex <==
\begin{tikzpicture}[decoration=snake]
\draw[black, rounded corners] (8, 0) rectangle +(2, 2); 
\path (8, 2) --  (8, 0) node[midway,left] {QPU$_\text{A}$};

\begin{scope}[every node/.style={fill, circle, minimum size=10pt}]
    \node (A) at (8.4, 1.6) {};
    \node (B) [right = 0.25 of A] {};
    \node (C) [fill = OliveGreen, right = 0.25 of B] {};
    \node (D) at (8.4, 1) {};
    \node (E) [right = 0.25 of D] {};
    \node (F) [right = 0.25 of E] {};
    \node (G) at (8.4, 0.4) {};
    \node (H) [right = 0.25 of G] {};
    \node (I) [fill = OliveGreen, right = 0.25 of H] {};
\end{scope}

\draw[black, rounded corners] (14, -2) rectangle +(2, 2); 
\path (14 + 2, 2 - 2) --  (14 + 2, -2) node[midway,right] {QPU$_\text{B}$};

\begin{scope}[every node/.style={fill, circle, minimum size=10pt}]
    \node (1) [fill = OliveGreen, ] at (14.4, -0.4) {};
    \node (2) [right = 0.25 of 1] {};
    \node (3) [right = 0.25 of 2] {};
    \node (4) at (14.4, -1) {};
    \node (5) [right = 0.25 of 4] {};
    \node (6) [right = 0.25 of 5] {};
    \node (7) [fill = OliveGreen, ] at (14.4, -1.6) {};
    \node (8) [right = 0.25 of 7] {};
    \node (9) [right = 0.25 of 8] {};
\end{scope}

\draw[decorate, thick, draw=OliveGreen] (C) --node[midway,above right] {$|\Phi^+\rangle$} (1);

\draw[black, rounded corners] (10, -4) rectangle +(2, 2); 
\path (10, - 4) --  (10 + 2, - 4) node[midway,below] {QPU$_\text{C}$};

\begin{scope}[every node/.style={fill, circle, minimum size=10pt}]
    \node (11) [fill = OliveGreen, ] at (10.4, -2.4) {};
    \node (12) [right = 0.25 of 11] {};
    \node (13) [fill = OliveGreen, right = 0.25 of 12] {};
    \node (14) at (10.4, -3) {};
    \node (15) [right = 0.25 of 14] {};
    \node (16) [right = 0.25 of 15] {};
    \node (17) at (10.4, -3.6) {};
    \node (18) [right = 0.25 of 17] {};
    \node (19) [right = 0.25 of 18] {};
\end{scope}

\draw[decorate, thick, draw=OliveGreen] (I) --node[midway, below left] {$|\Phi^+\rangle$} (11);
\draw[decorate, thick, draw=OliveGreen] (7) --node[midway, below right] {$|\Phi^+\rangle$} (13);

\draw [black, double] plot [smooth, tension=0] coordinates { (9, 0) (9, -3) (10, -3)};
\draw [black, double] plot [smooth, tension=0] coordinates { (12, -3) (15, -3) (15, -2)};
\draw [black, double] plot [smooth, tension=0] 
coordinates { (9, 2) (9, 2.5) (15, 2.5) (15, 0)};
\end{tikzpicture}
